A computational study of how surfaces affect slip family activity

Plastic deformation behavior is most conveniently assessed by characterization on a surface, but whether such observations are representative of bulk properties is uncertain. Motivated by reported inconsistencies in slip resistance probed at different depths, we investigated (i) whether the average slip family activity is affected by the presence of a surface and (ii) how the kinematic nature of available slip families influences a potential surface effect. The slip family activity as a function of distance from the surface was extracted from full-field crystal plasticity simulations of random polycrystalline hexagonal close-packed (HCP) and body-centered cubic (BCC) metals as examples of mixed in contrast to universally-high numbers of slip systems per family. Under certain conditions, a deviation from bulk slip activity is observed up to about two grains from the surface. For the easiest (least slip-resistant) family, a surface effect of decreasing activity with depth emerges if the number of slip systems falls below about six. For harder families, slip activity always increases with depth. These phenomena are explained on the basis of varying constraints with depth in connection with the kinematic properties of slip families in the material.

==> abstract.tex <==
Plastic deformation behavior is most conveniently assessed by characterization on a surface, but whether such observations are representative of bulk properties is uncertain. 
Motivated by reported inconsistencies in slip resistance probed at different depths, we investigated (i) whether the average slip family activity is affected by the presence of a surface and (ii) how the kinematic nature of available slip families influences a potential surface effect.
The slip family activity as a function of distance from the surface was extracted from full-field crystal plasticity simulations of random polycrystalline hexagonal close-packed (HCP) and body-centered cubic (BCC) metals as examples of mixed in contrast to universally-high numbers of slip systems per family.
Under certain conditions, a deviation from bulk slip activity is observed up to about two grains from the surface.
For the easiest (least slip-resistant) family, a surface effect of decreasing activity with depth emerges if the number of slip systems falls below about six. 
For harder families, slip activity always increases with depth.
These phenomena are explained on the basis of varying constraints with depth in connection with the kinematic properties of slip families in the material.

==> config.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
% \usepackage[square,numbers]{natbib}
\usepackage{fourier}
\usepackage{textcomp}
\usepackage{textalpha}
\usepackage{verbatim}
\usepackage{etoolbox}
\usepackage{xinttools}
\usepackage{xspace} % to get the spacing after macros right  
\usepackage[dvipsnames,svgnames]{xcolor}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{siunitx}
\usepackage{miller}
\usepackage{subfig}
\usepackage{subeqnarray}
\usepackage{multirow}
\usepackage{tabularray}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage[normalem]{ulem}
\usepackage{graphbox}
\usepackage{enumitem} % for changing lists (especially the vertical spacing)
\usepackage{calc}
\usepackage{todonotes}
\usepackage{color,soul}
\usepackage{hyperref}

\hypersetup{
    colorlinks = true,
    allcolors = NavyBlue,
    bookmarksnumbered=true,
    %pagebackref=true,
    pdfpagelabels=false,
    plainpages = false,
}
\usepackage[capitalize]{cleveref}
% \usepackage{doi}

\graphicspath{{./}{./figures}}
\DeclareGraphicsExtensions{.pdf,.png}

\sisetup{
 list-units=single,
 list-final-separator={,\ \text{and}\ },
 separate-uncertainty=true,
 }

\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4} 
\setcounter{dbltopnumber}{2}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\textfraction}{0.05}
\renewcommand{\floatpagefraction}{0.7}
\renewcommand{\dblfloatpagefraction}{0.7}


% NEW COMMANDS
\newcommand{\upalpha}{\ensuremath{\text{\textalpha}}}
\newcommand{\latin}[1]{\textit{#1}}
\newcommand{\pcnt}[1]{\SI{#1}{\percent}}

\newcommand{\Revision}[2][]{\textcolor{BrickRed}{\sout{#1}}\textcolor{BurntOrange}{#2}}
\newcommand{\Added}[1]{\textcolor{BurntOrange}{#1}} 
\newcommand{\Deleted}[1]{\textcolor{red}{\sout{#1}}} 
\newcommand{\Note}[1]{\textcolor{CornflowerBlue}{#1}}
\newcommand{\Question}[1]{\textcolor{Red}{#1?}}
\newcommand{\Answer}[1]{\textcolor{LimeGreen}{#1}}

\definecolor{basal}{RGB}{0, 0, 255}
\definecolor{prism}{RGB}{255, 0, 0}
\definecolor{pyrca}{RGB}{245, 155, 0}

\newcommand{\distance}{\ensuremath{d}}
\newcommand{\dist}[1][]{\ensuremath{D_\text{#1}}}
\newcommand{\Ngrain}{\ensuremath{n_\text{grain}}\xspace}
\newcommand{\Ngrid}{\ensuremath{N}\xspace}
\newcommand{\Dnorm}{\ensuremath{D_\text{grain}}\xspace}
\newcommand{\dgrain}{\ensuremath{d_\text{grain}}\xspace}



% CRYSTALLOGRAPHY

\newcommand{\crystaxis}[1]{\ensuremath{\langle{#1}\rangle}}


\newcommand{\basalA}{\ensuremath{\text{basal}\,\crystaxis{a}}\xspace}
\newcommand{\prismA}{\ensuremath{\text{prismatic}\,\crystaxis{a}}\xspace}
\newcommand{\pyrCA}{\ensuremath{\text{pyramidal}\,\crystaxis{c+a}}\xspace}


% CONSTITUTIVE LAW
\newcommand{\caratio}{\ensuremath{c/a} ratio}
\newcommand{\slipresistance}[1][]{\ensuremath{\xi^{#1}}}
\newcommand{\slipresistancerate}[1][]{\ensuremath{\dot{\xi}^{#1}}}
\newcommand{\initialresistance}[1][]{\ensuremath{\xi_0^{#1}}}
\newcommand{\finalresistance}[1][]{\ensuremath{\xi_\infty^{#1}}}
\newcommand{\hardeningref}{\ensuremath{h_0}}
\newcommand{\slipsysteminteraction}[1][]{\ensuremath{h_{#1}}}
\newcommand{\hardeningexp}{\ensuremath{a}}
\newcommand{\rss}[1][]{\ensuremath{\tau^{#1}}}
\newcommand{\slipdirection}[1][]{\ensuremath{\vctr{m}^{#1}}}
\newcommand{\slipplane}[1][]{\ensuremath{\vctr{n}^{#1}}}
\newcommand{\shearrate}[1][]{\ensuremath{\dot\gamma^{#1}}}
\newcommand{\shearrateref}{\ensuremath{\shearrate_0}}
\newcommand{\stressexp}{\ensuremath{n}}
\newcommand{\Taylorfactor}{\ensuremath{M}}


% ABBREVIATIONS

\newcommand{\ie}{\latin{i.\hspace{1pt}e.}\xspace}
\newcommand{\eg}{\latin{e.\hspace{1pt}g.}\xspace}
\newcommand{\aka}{\latin{a.\hspace{1pt}k.\hspace{1pt}a.}\xspace}
\newcommand{\etc}{\latin{etc.}\xspace}
\newcommand{\cf}{\latin{cf.}\xspace}


% NAMES 

\newcommand{\term}[1]{#1\xspace}
\newcommand{\Eshelby}{\term{Eshelby}}
\newcommand{\Euler}{\term{Euler}}
\newcommand{\Gauss}{\term{Gauss}}
\newcommand{\KN}{\term{Kr\"oner}--\term{Nye}}
\newcommand{\PK}{\term{Piola}--\term{Kirchhoff}}
\newcommand{\Cauchy}{\term{Cauchy}}
\newcommand{\Burgers}{\term{Burgers}}
\newcommand{\Mandel}{\term{Mandel}}
\newcommand{\NR}{\term{Newton}--\term{Raphson}}
\newcommand{\Frobenius}{\term{Frobenius}}
\newcommand{\RK}{\term{Runge}--\term{Kutta}}
\newcommand{\Orowan}{\term{Orowan}}
\newcommand{\Schmid}{\term{Schmid}}
\newcommand{\Miller}{\term{Miller}}


% PHYSICAL CONSTANTS

\newcommand{\kB}{k_\text{B}}



% TENSORS 

\newcommand{\field}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\tnsr}[1]{\ensuremath{\vb{#1}}}
\newcommand{\vctr}[1]{\ensuremath{\vb{#1}}}


% FUNCTIONS AND OPERATORS

\newcommand{\transpose}[1]{\ensuremath{{#1}^{\text T}}}
\newcommand{\inverse}[1]{\ensuremath{{#1}^{-1}}}
\newcommand{\invtranspose}[1]{\ensuremath{{#1}^{\text{-T}}}}
\newcommand{\sign}[1]{\ensuremath{\operatorname{sign}{#1}}}
\newcommand{\signb}[1]{\ensuremath{\operatorname{sign}\left({#1}\right)}}
\newcommand{\act}{}
\newcommand{\dblCont}{:}


% SPECIAL TENSORS

\newcommand{\identity}{\tnsr I}
\newcommand{\levi}{\ensuremath{\epsilon}}


% VARIABLES

\newcommand{\SF}{\ensuremath{m}}
\newcommand{\LRB}{\ensuremath{M}}
\newcommand{\LM}{\ensuremath{m^\prime}}

\newcommand{\stiffness}{\ensuremath{\field C}}
\newcommand{\F}{\ensuremath{\tnsr F}}
\newcommand{\Fdot}[1][]{\ensuremath{\dot{\tnsr F}_\text{#1}}}
\newcommand{\Fdotcomp}[1]{\ensuremath{\dot F_{#1}}}
\newcommand{\Fp}{\ensuremath{\tnsr F_\text{p}}}
\newcommand{\Fpdot}{\ensuremath{\dot{\tnsr F}_\text{p}}}
\newcommand{\Fi}{\ensuremath{\tnsr F_\text{i}}}
\newcommand{\Fidot}{\ensuremath{\dot{\tnsr F}_\text{i}}}
\newcommand{\Fe}{\ensuremath{\tnsr F_\text{e}}}
\newcommand{\Lp}{\ensuremath{\tnsr L_\text{p}}}
\newcommand{\Li}{\ensuremath{\tnsr L_\text{i}}}
\newcommand{\E}{\ensuremath{\tnsr E}}
\newcommand{\GL}{\ensuremath{\tnsr E_\text{e}}}
\newcommand{\cauchy}{\ensuremath{\tnsrgreek \sigma}}
\newcommand{\fPK}[1][]{\ensuremath{{\tnsr P}_\text{#1}}}
\newcommand{\sPK}{\ensuremath{\tnsr S}}
\newcommand{\Mp}{\ensuremath{\tnsr M_\text{p}}}
\newcommand{\Mi}{\ensuremath{\tnsr M_\text{i}}}
\newcommand{\shear}{\ensuremath{\gamma}}
\newcommand{\strain}{\ensuremath{\varepsilon}}
\newcommand{\orientation}{\ensuremath{\tnsr O}}
\newcommand{\rotation}{\ensuremath{\tnsr R}}
\newcommand{\stretchtensor}{\ensuremath{\tnsr U}}
\newcommand{\elasticity}{\ensuremath{E}}


% xi row name
\newcommand{\twoonefour}{1 (2:1:4)\xspace}
\newcommand{\onetwofour}{2 (1:2:4)\xspace}
\newcommand{\onefourfour}{3 (1:4:4)\xspace}
\newcommand{\onetwotwo}{4 (1:2:2)\xspace}
\newcommand{\twotwoone}{5 (2:2:1)\xspace}
\newcommand{\oneoneone}{6 (1:1:1)\xspace}
\newcommand{\oneonetwo}{7 (1:1:2)\xspace}
\newcommand{\oneonefour}{8 (1:1:4)\xspace}

\newcommand{\onetwo}{1 (1:2)\xspace}
\newcommand{\oneonepone}{2 (1:1.1)\xspace}
\newcommand{\oneone}{3 (1:2)\xspace}
\newcommand{\oneponeone}{4 (1.1:1)\xspace}
\newcommand{\twoone}{5 (2:1)\xspace}


% NEW UNITS 

\DeclareSIUnit\micron{\micro\metre}

%plot
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\newcommand{\convsize}{1.2in}
\newsavebox{\measurebox}

==> frontmatter_Elsevier.tex <==
\begin{frontmatter}
 \title{\input{title}}


\author[MSU_PA]{Cathy Bing}
\ead{zhangrux@msu.edu}

\author[MSU_CHEMS]{Thomas R. Bieler}
\ead{bieler@egr.msu.edu}

\author[MSU_CHEMS]{Philip Eisenlohr\corref{PE}}
\ead{eisenlohr@egr.msu.edu}

\cortext[PE]{Corresponding author}

\affiliation[MSU_PA]{
                organization={Physics and Astronomy, 
                              Michigan State University},
%                addressline={Jawahar Nagar}, 
                city={East Lansing},
%               citysep={},
                state={MI},
                statesep={}, 
                postcode={48824}, 
                country={USA}}

\affiliation[MSU_CHEMS]{
                organization={Chemical Engineering and Materials Science, 
                              Michigan State University},
%                addressline={Jawahar Nagar}, 
                city={East Lansing},
%               citysep={},
                state={MI},
                statesep={}, 
                postcode={48824}, 
                country={USA}}

\begin{abstract}
    \input{abstract}
\end{abstract}
\begin{keyword}
    \input{keywords}
\end{keyword}
\end{frontmatter}


==> frontmatter_Springer.tex <==
\setcitestyle{numbers,square}

\title{\input{title}}
%\titlerunning{Short form of title}

\author{
Cathy Bing
\and Thomas R. Bieler
\and Philip Eisenlohr
}
%\authorrunning{Short form of author list}

\institute{
Cathy Bing
\at
Physics and Astronomy,
Michigan State University,
East Lansing, MI 48824, USA \\
\email{zhangrux@msu.edu}
\and
Thomas R. Bieler
\and Philip Eisenlohr
\at
Chemical Engineering and Materials Science,
Michigan State University,
East Lansing, MI 48824, USA \\
Tel.: +1 (517) 432-4506\\
\email{pe@msu.edu}
}

\date{Received: \today\ / Accepted: date}

\maketitle

\begin{abstract}
\input{abstract}
\def\sep{,}
\keywords{
\input{keywords}
}
\end{abstract}


==> keywords.tex <==
surface effect%
\xspace\sep\xspace
slip family kinematics and multiplicity%
\xspace\sep\xspace
crystal plasticity simulation%


==> title.tex <==
A computational study of how surfaces affect slip family activity

